Tangent cones of Hermitian Yang-Mills connections with isolated singularities

We give a simple direct proof of uniqueness of tangent cones for singular projectively Hermitian Yang-Mills connections on reflexive sheaves at isolated singularities modelled on $\mu$-polystable holomorphic bundles over $\mathbf{P}^{n-1}$.

==> pre/colors.tex <==
\usepackage{multicol, color}

\definecolor{gold}{rgb}{0.85,.66,0}
\definecolor{cherry}{rgb}{0.9,.1,.2}
\definecolor{burgundy}{rgb}{0.8,.2,.2}
\definecolor{orangered}{rgb}{0.85,.3,0}
\definecolor{orange}{rgb}{0.85,.4,0}
\definecolor{olive}{rgb}{.45,.4,0}
\definecolor{lime}{rgb}{.6,.9,0}
%\definecolor{green}{rgb}{.3,.5,0}
\definecolor{green}{rgb}{.2,.7,0}
\definecolor{grey}{rgb}{.4,.4,.2}
\definecolor{brown}{rgb}{.4,.3,.1}
\def\gold#1{\textcolor{gold}{#1}}
\def\cherry#1{\textcolor{cherry}{#1}}
\def\burgundy#1{\textcolor{burgundy}{#1}}
\def\orange#1{\textcolor{orange}{#1}}
\def\orangered#1{\textcolor{orangered}{#1}}
\def\olive#1{\textcolor{olive}{#1}}
\def\lime#1{\textcolor{lime}{#1}}
\def\green#1{\textcolor{green}{#1}}
\def\grey#1{\textcolor{grey}{#1}}
\def\brown#1{\textcolor{brown}{#1}}


==> pre/conf.tex <==
\newif\ifpaper
\newif\ifarxiv

\paperfalse
\arxivfalse
% \papertrue
% \arxivtrue


==> pre/init.tex <==
\usepackage{etoolbox}
\newtoggle{arXiv}
\newtoggle{screen}
